Minimal Intervention Shared Control with Guaranteed Safety under Non-Convex Constraints

Shared control combines human intention with autonomous decision-making. At the low level, the primary goal is to maintain safety regardless of the user's input to the system. However, existing shared control methods-based on, e.g., Model Predictive Control, Control Barrier Functions, or learning-based control-often face challenges with feasibility, scalability, and mixed constraints. To address these challenges, we propose a Constraint-Aware Assistive Controller that computes control actions online while ensuring recursive feasibility, strict constraint satisfaction, and minimal deviation from the user's intent. It also accommodates a structured class of non-convex constraints common in real-world settings. We leverage Robust Controlled Invariant Sets for recursive feasibility and a Mixed-Integer Quadratic Programming formulation to handle non-convex constraints. We validate the approach through a large-scale user study with 66 participants-one of the most extensive in shared control research-using a simulated environment to assess task load, trust, and perceived control, in addition to performance. The results show consistent improvements across all these aspects without compromising safety and user intent. Additionally, a real-world experiment on a robotic manipulator demonstrates the framework's applicability under bounded disturbances, ensuring safety and collision-free operation.

==> images/problem_formulation/polytopes/environment.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=0.4]

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
hide x axis,
hide y axis,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-6, xmax=6,
xtick style={color=black},
y grid style={darkgray176},
ymin=-4, ymax=4,
ytick style={color=black}
]
\path [draw=black, thick]
(axis cs:2,2.41421356237309)
--(axis cs:3.41421356237309,1)
--(axis cs:2,-0.414213562373095)
--(axis cs:0.585786437626905,1)
--cycle;


\path [draw=black, thick]
(axis cs:-5. , -3.)
--(axis cs:-5.,  3.)
--(axis cs:5., 3.)
--(axis cs:5.,  -3.)
--cycle;
\path [draw=black, thick]
(axis cs:-4,-2.5)
--(axis cs:-2,-2.5)
--(axis cs:-3,0.5)
--cycle;
\draw (axis cs:1.5,1) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$n_b ={1}$};
\draw (axis cs:-3.5,-1.5) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$n_b ={2}$};
\end{axis}

\end{tikzpicture}


==> images/problem_formulation/polytopes/polytopes.tex <==
\begin{tikzpicture}[scale=0.6]
    % Top figure (single)
    \node (top) at (0,3.6) {\input{images/problem_formulation/polytopes/environment}};

    % Bottom left figure
    \node (left) at (-2.2,0) {\input{images/problem_formulation/polytopes/rhombus}};

    % Bottom right figure
    \node (right) at (2.2,0) {\input{images/problem_formulation/polytopes/triangle}};

    % Arrows from top figure to bottom figures
    \draw[-, thick, densely dotted] (0,2.05) -- (0,1.9);
    \draw[-, thick, densely dotted] (0,1.9) -- (-2.2,1.9);
    \draw[->, thick, densely dotted] (-2.2,1.9) -- (-2.2,1.5);
    \draw[-, thick, densely dotted] (0,1.9) -- (2.2,1.9);
    \draw[->, thick, densely dotted] (2.2,1.9) -- (2.2,1.5);
\end{tikzpicture}

==> images/problem_formulation/polytopes/rhombus.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=0.4]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{yellow}{RGB}{255,255,0}

\begin{axis}[
hide x axis,
hide y axis,
legend cell align={left},
legend columns=2,
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1,1.22)},
  anchor=south west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-6, xmax=6,
xtick style={color=black},
y grid style={darkgray176},
ymin=-4, ymax=4,
ytick style={color=black}
]
\path [draw=black, thick]
(axis cs:2,2.41421356237309)
--(axis cs:3.41421356237309,1)
--(axis cs:2,-0.414213562373095)
--(axis cs:0.585786437626905,1)
--cycle;
\path [draw=black, fill=red, opacity=0.2, thick, postaction={pattern=north west lines, fill opacity=0.2}]
(axis cs:5,-0.585786437626905)
--(axis cs:5,3)
--(axis cs:1.41421356237309,3)
--cycle;
\addlegendimage{area legend, draw=black, fill=red, opacity=0.2, thick, postaction={pattern=north west lines, fill opacity=0.2}}
\addlegendentry{polytopes 0}

\path [draw=black, fill=blue, opacity=0.2, thick, postaction={pattern=vertical lines, fill opacity=0.2}]
(axis cs:-0.585786437626905,-3)
--(axis cs:5,-3)
--(axis cs:5,2.58578643762691)
--cycle;
\addlegendimage{area legend, draw=black, fill=blue, opacity=0.2, thick, postaction={pattern=vertical lines, fill opacity=0.2}}
\addlegendentry{polytopes 1}

\path [draw=black, fill=green, opacity=0.2, thick, postaction={pattern=north east lines, fill opacity=0.2}]
(axis cs:-5,-3)
--(axis cs:4.58578643762691,-3)
--(axis cs:-1.41421356237309,3)
--(axis cs:-5,3)
--cycle;
\addlegendimage{area legend, draw=black, fill=green, opacity=0.2, thick, postaction={pattern=north east lines, fill opacity=0.2}}
\addlegendentry{polytopes 2}

\path [draw=black, fill=yellow, opacity=0.2, thick, postaction={pattern=horizontal lines, fill opacity=0.2}]
(axis cs:-5,-3)
--(axis cs:-3.41421356237309,-3)
--(axis cs:2.58578643762691,3)
--(axis cs:-5,3)
--cycle;
\addlegendimage{area legend, draw=black, fill=yellow, opacity=0.2, thick, postaction={pattern=horizontal lines, fill opacity=0.2}}
\addlegendentry{polytopes 3}

\path [draw=black, thick]
(axis cs:-5. , -3.)
--(axis cs:-5.,  3.)
--(axis cs:5., 3.)
--(axis cs:5.,  -3.)
--cycle;

\path [draw=black, thick, dashed]
(axis cs:5,-0.585786437626905)
--(axis cs:5,3)
--(axis cs:1.41421356237309,3)
--cycle;
\path [draw=black, thick, dashed]
(axis cs:-0.585786437626905,-3)
--(axis cs:5,-3)
--(axis cs:5,2.58578643762691)
--cycle;
\path [draw=black, thick, dashed]
(axis cs:-5,-3)
--(axis cs:4.58578643762691,-3)
--(axis cs:-1.41421356237309,3)
--(axis cs:-5,3)
--cycle;
\path [draw=black, thick, dashed]
(axis cs:-5,-3)
--(axis cs:-3.41421356237309,-3)
--(axis cs:2.58578643762691,3)
--(axis cs:-5,3)
--cycle;
\draw (axis cs:3.00473785412437,2.30473785412437) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(1,0)$};
\draw (axis cs:3.0380711874577,-.880711874577) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(1,1)$};
\draw (axis cs:-2.80710678118655,0) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(1,2)$};
\draw (axis cs:-1.50710678118655,-2) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(1,3)$};
\legend{}
\end{axis}
\end{tikzpicture}


==> images/problem_formulation/polytopes/triangle.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=0.4]

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
hide x axis,
hide y axis,
legend cell align={left},
legend columns=2,
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1,1.22)},
  anchor=south west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-6, xmax=6,
xtick style={color=black},
y grid style={darkgray176},
ymin=-4, ymax=4,
ytick style={color=black}
]
\path [draw=black, thick]
(axis cs:-4,-2.5)
--(axis cs:-2,-2.5)
--(axis cs:-3,0.5)
--cycle;
\path [draw=black, fill=red, opacity=0.2, thick, postaction={pattern=north west lines, fill opacity=0.2}]
(axis cs:-5,-3)
--(axis cs:5,-3)
--(axis cs:5,-2.5)
--(axis cs:-5,-2.5)
--cycle;
\addlegendimage{area legend, draw=black, fill=red, opacity=0.2, thick, postaction={pattern=north west lines, fill opacity=0.2}}
\addlegendentry{polytopes 0}

\path [draw=black, fill=blue, opacity=0.2, thick, postaction={pattern=vertical lines, fill opacity=0.2}]
(axis cs:-1.83333333333333,-3)
--(axis cs:5,-3)
--(axis cs:5,3)
--(axis cs:-3.83333333333333,3)
--cycle;
\addlegendimage{area legend, draw=black, fill=blue, opacity=0.2, thick, postaction={pattern=vertical lines, fill opacity=0.2}}
\addlegendentry{polytopes 1}

\path [draw=black, fill=green, opacity=0.2, thick, postaction={pattern=north east lines, fill opacity=0.2}]
(axis cs:-5,-3)
--(axis cs:-4.16666666666667,-3)
--(axis cs:-2.16666666666667,3)
--(axis cs:-5,3)
--cycle;
\addlegendimage{area legend, draw=black, fill=green, opacity=0.2, thick, postaction={pattern=north east lines, fill opacity=0.2}}
\addlegendentry{polytopes 2}

\path [draw=black, thick]
(axis cs:-5. , -3.)
--(axis cs:-5.,  3.)
--(axis cs:5., 3.)
--(axis cs:5.,  -3.)
--cycle;

\path [draw=black, thick, dashed]
(axis cs:-5,-3)
--(axis cs:5,-3)
--(axis cs:5,-2.5)
--(axis cs:-5,-2.5)
--cycle;
\path [draw=black, thick, dashed]
(axis cs:-1.83333333333333,-3)
--(axis cs:5,-3)
--(axis cs:5,3)
--(axis cs:-3.83333333333333,3)
--cycle;
\path [draw=black, thick, dashed]
(axis cs:-5,-3)
--(axis cs:-4.16666666666667,-3)
--(axis cs:-2.16666666666667,3)
--(axis cs:-5,3)
--cycle;
\draw (axis cs:-3.5,-2.80) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(2,0)$};
\draw (axis cs:0.583333333333333,0) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(2,1)$};
\draw (axis cs:-4.78333333333333,0) node[
  scale=0.5,
  fill=white,
  draw=black,
  line width=0.4pt,
  inner sep=4pt,
  fill opacity=1.0,
  anchor=base west,
  text=black,
  rotate=0.0
]{$P_{D}(2,2)$};
\legend{}
\end{axis}

\end{tikzpicture}


==> images/problem_formulation/test.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green}{RGB}{0,128,0}
\definecolor{green01270}{RGB}{0,127,0}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-6, xmax=6,
xtick style={color=black},
y grid style={darkgray176},
ymin=-4, ymax=4,
ytick style={color=black}
]
\path [draw=black, thick]
(axis cs:-4,-2.5)
--(axis cs:-2,-2.5)
--(axis cs:-3,0.5)
--cycle;
\path [draw=black, fill=red, opacity=0.2, thick, postaction={pattern=crosshatch, fill opacity=0.2}]
(axis cs:-5,-3)
--(axis cs:5,-3)
--(axis cs:5,-2.5)
--(axis cs:-5,-2.5)
--cycle;
\path [draw=black, fill=blue, opacity=0.2, thick, postaction={pattern=crosshatch dots, fill opacity=0.2}]
(axis cs:-1.83333333333333,-3)
--(axis cs:5,-3)
--(axis cs:5,3)
--(axis cs:-3.83333333333333,3)
--cycle;
\path [draw=black, fill=green, opacity=0.2, thick, postaction={pattern=fivepointed stars, fill opacity=0.2}]
(axis cs:-5,-3)
--(axis cs:-4.16666666666667,-3)
--(axis cs:-2.16666666666667,3)
--(axis cs:-5,3)
--cycle;
\addplot [semithick, red, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-2.16666666666667 3
};
\addplot [semithick, red, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
5 -2.5
};
\addplot [semithick, red, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-4.16666666666667 -3
};
\addplot [semithick, red, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-1.83333333333333 -3
};
\addplot [semithick, red, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-3.83333333333333 3
};
\addplot [semithick, red, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-5 -2.5
};
\addplot [semithick, blue, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
5 -3
};
\addplot [semithick, blue, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
5 3
};
\addplot [semithick, blue, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-5 -3
};
\addplot [semithick, blue, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-5 3
};
\addplot [semithick, green01270, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
5 3
};
\addplot [semithick, green01270, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
5 -3
};
\addplot [semithick, green01270, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-5 3
};
\addplot [semithick, green01270, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
-5 -3
};
\end{axis}

\end{tikzpicture}


==> tables/robustness_analysis.tex <==
% \begin{table*}
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|ccc}
% \toprule
No. of Trials & Success & Model Disturbance & delay (sec)  \\
\midrule
3 & & - & - \\
3 & & $\overline{[1, 0.1, 1, 0.1]^{\top}}$ & - \\
3 & & $\overline{[3, 0.2, 3, 0.2]^{\top}}$ & - \\
3 & & $\overline{[1, 0.1, 1, 0.1]^{\top}}$ & $1$sec \\
3 & & $\overline{[3, 0.2, 3, 0.2]^{\top}}$ & $3$sec \\
\bottomrule
\end{tabular}
% \caption{
% Test results for robustness and teleoprtation delay.}
% \label{tab:robust_analysis}
% \figvspace{}
% \end{table*}
